Pilotfish: Distributed Execution for Scalable Blockchains

Scalability is a crucial requirement for modern large-scale systems, enabling elasticity and ensuring responsiveness under varying load. While cloud systems have achieved scalable architectures, blockchain systems remain constrained by the need to over-provision validator machines to handle peak load. This leads to resource inefficiency, poor cost scaling, and limits on performance. To address these challenges, we introduce Pilotfish, the first scale-out transaction execution engine for blockchains. Pilotfish enables validators to scale horizontally by distributing transaction execution across multiple worker machines, allowing elasticity without compromising consistency or determinism. It integrates seamlessly with the lazy blockchain architecture, completing the missing piece of execution elasticity. To achieve this, Pilotfish tackles several key challenges: ensuring scalable and strongly consistent distributed transactions, handling partial crash recovery with lightweight replication, and maintaining concurrency with a novel versioned-queue scheduling algorithm. Our evaluation shows that Pilotfish scales linearly up to at least eight workers per validator for compute-bound workloads, while maintaining low latency. By solving scalable execution, Pilotfish brings blockchains closer to achieving end-to-end elasticity, unlocking new possibilities for efficient and adaptable blockchain systems.

==> sections/conclusion.tex <==
\section{Conclusion}
\sysname is the first blockchain execution engine allowing a blockchain validator to harness multiple machines under its control to horizontally scale execution. \sysname supports dynamic reads and writes, thus supporting programming models where the input read and write set is only partially specified by the transaction. \sysname also tolerates crash-faults internal to the validator and provably satisfies serializability, determinism, and liveness.
Our implementation of \sysname demonstrates scalability under varying system loads, showing it outperforms the baseline Sui execution engine by up to 8x under heavy CPU loads.

==> sections/extensions.tex <==
\section{Going Further: Fault Tolerance and Dynamic Accesses}\label{sec:extensions}

The basic protocol in the previous section relies on two assumptions: (1) that workers do not fail, and (2) that transactions' read and write sets are known in advance. In the full \sysname protocol, we remove these assumptions. Due to space limitations, we provide a high-level summary of our approach in this section; Appendices~\ref{sec:cft}--\ref{sec:child-details} contain detailed explanations, pseudocode and proofs.

To ensure robust crash fault tolerance despite inevitable component failures, \sysname employs a replication architecture by dedicating multiple machines to each \execworker. \sysname makes the key insight that in our setting replication can provide strong consistency without using a consensus protocol between workers. This is because the blockchain's commit sequence already provides a permanent and globally available order of transactions, so there is no need for workers to run consensus to agree on this order again. Based on this insight, we design a lightweight replication mechanism that only employs minimal communication between replicas of the same logical \execworker. To recover from crashes, a range of recovery procedures are available, depending on the number of crashes and how out-of-sync replicas are with respect to each other: from a simple reconfiguration scheme (peers of a crashed replica simply start communicating with another replica and continue executing seamlessly) to full external recovery (syncing checkpointed state from another validator and re-executing all transactions after that checkpoint).

To support transactions that only partially specify their read/write sets, \sysname introduces a mechanism for handling parent-child object relationships where child objects are dynamically accessed during execution. Transactions must include the root (parent) object, and access to child objects is permitted if the root is part of the transaction. To manage dynamic discovery of child objects while maintaining parallelism, \sysname treats each version of an object as a new object, creating separate queues per (\objectid,\objectversion), which allows independent progress of different versions and resolves false sharing. To prevent inconsistencies from out-of-order writes, it buffers writes to ensure they are written to disk in order. When a transaction discovers new child objects during execution, it halts and generates an augmented transaction \txaugmented that includes the newly discovered child objects in its read and write sets. This process continues until all necessary child objects are included, allowing the transaction to proceed to successful execution without prior overprediction of its read/write sets.

==> sections/intro-old.tex <==
\section{Introduction} \label{sec:introduction}
% What we do
% For many essential online services, blockchains are a decentralized, secure and privacy-preserving alternative to centralized cloud-based solutions. One obstacle to mass adoption of blockchain for these services is \textit{scalability}: the blockchain must be able to serve requests in a timely manner, even as the load increases.

Despite a decade of research by the secure distributed computing community~\cite{byzcoin, omniledger, elastico, bitcoinng, chainspace, dumbo-ng, bullshark, narwhal, hotstuff, jolteon, mysticeti}, blockchains are far from able to compete with centralized solutions.
% Scaling blockchain protocols to support the global economy has been at the forefront of secure distributed systems research for a decade now~\cite{byzcoin, omniledger, elastico, bitcoinng, chainspace, dumbo-ng, bullshark, narwhal, hotstuff, jolteon}. Yet, current solutions are still far from able to compete with centralized cloud-based services. 
Ethereum is almost always congested, often pushing transaction fees into the tens of USD\footnote{\url{https://bitinfocharts.com/comparison/ethereum-transactionfees.html\#3y}}.
Base, a promising Layer 2 solution that is built by prominent exchange Coinbase suffered severe congestion when pushed to have more than 1 million transactions in a day\footnote{\url{https://finance.yahoo.com/news/l2-network-congestion-causing-transactions-045758034.html}}.
The main obstacle currently is that of scalable transaction execution.

One straightforward approach to scalability is that of vertical scalability: executing blockchain transactions in parallel on each validator machine, thus fully leveraging the available CPU cores. This approach has the advantage of resource efficiency, but it also has limitations. First, it has a single-machine performance ceiling: there is a limit to how powerful a single validator machine can be, meaning that validator performance cannot scale past a certain level. Second, it does not provide \textit{elasticity}: the (hardware) resource use and costs of validators does not scale with the load; instead, validators have to overprovision their machines so as to be able to handle high-load scenarios.
For instance, the requirements to run a Solana validator are high: at least 16 CPU cores and 512GB of RAM\footnote{https://docs.solanalabs.com/operations/requirements}. And yet to this day, Solana suffers from both yearly incidents and congestion\footnote{\url{https://dailycoin.com/why-are-solana-transactions-failing-devs-scramble-to-fix-it/}}.
As a result, the vertical scaling solution (1) requires heavy upfront investment and maintenance costs and (2) still fails to deliver good user experience. At low load the validators are operating at a loss, and at high load users are not getting a fair market price for their transactions (as supply does not scale with demand).

In summary, the current Web3 experience is far from the simplicity and performance of cloud services, and as a result users choose to risk their data and security in centralized services.
We therefore argue that blockchain systems should provide both elasticity and scalability.
% Finally, Solana, the first blockchain to focus on parallel execution fully leveraging validators' available CPU cores, 
% These issues are present even as validators are no longer using low-end commodity machines. For instance, the requirements to run a Solana validator are high: at least 16 CPU cores and 512GB of RAM\footnote{https://docs.solanalabs.com/operations/requirements}. 

% The key reason why this happens is because existing blockchains are not \emph{elastic}. 
%They require big upfront costs from validators who operate at a loss  until the blockchain becomes popular at which point the user experience is compromised due to high costs, as it is no longer a supply-demand market, and extremely high transaction latencies.

One potential solution for elastic blockchain scalability is inter-validator sharding~\cite{omniledger,chainspace,avarikioti2023divide, byzcuit}. In these systems the blockchain state is split into shards as the load increases, with a subset of the validators handling each shard in parallel.
This is not only of academic interest, as the NEAR blockchain has launched a functional inter-validator sharding solution\footnote{https://medium.com/nearprotocol/phase-2-of-near-sharding-launches-dc1720304901}
which is an indication that elastic scalability can provide low costs and avoid congestion. However, these state sharding protocols have significant shortcomings related to security and ease of development. Firstly, sharding requires a sampling process from a bigger population of validators to subsets of validators per shard. These systems are thus less robust to adversarial attacks. For example Omniledger~\cite{omniledger} assumed a 25\% Byzantine adversary in order to provide sufficient 34\% security in all the sub-sampled shards. In the same vein, the adversary's adaptivity should be limited to once an epoch, as otherwise the adversary could target all its power in a single shard and compromise it. Finally, sharding is also challenging for user experience as there is significant fragmentation of the state. Transactions that need to span across multiple shards cost more and require expensive and slow atomic commit protocols~\cite{byzcuit}. %As a result this give an additional burden to developers who need to make sure they minimize such interactions. 

Lazy blockchains~\cite{celestia, lazyledger, prism,stefoexecuting, narwhal, bullshark, snap-and-chat, ebb-and-flow, mysticeti, dumbo-ng} take a different approach to elastic scaling, by separating the problems of data dissemination, consensus, and execution. A potentially distributed external~\cite{celestia,ebb-and-flow,lazyledger} or dedicated~\cite{prism, narwhal, snap-and-chat} subsystem acts as data-dissemination layer to receive client transactions, persist them as \emph{batches} of transactions, and disseminate them to other validators.
Each validator contains a single \emph{\primary} component running Byzantine agreement to sequence the digests of these batches. As a result, transaction data may be scattered across multiple machines (that we call \emph{\seqworkers}) and consensus is only achieved on metadata. This architecture provides elastic scaling to the problems of data-dissemination and ordering: if there is higher load, the system simply spins up more workers.
% If there is higher load, a lazy blockchain can spin-up more workers to handle the load while maintaining low fees and still making a profit. 
% In essence, it is the first blockchain that creates an efficient market. 
However, the elastic scalability stops at the ordering stage: existing lazy blockchains leave the retrieval of transactions from the \seqworkers and their execution as open problems~\cite{narwhal,bullshark}.


% Why current solutions fall short
%To the best of our knowledge, there exists no execution engine tackling these problems without crippling the system's performance and scalability.
Existing blockchains' execution engines are designed to run on a single machine that holds all the transaction data required for execution. Thus, when operating on top of a lazy blockchain, they need to fetch all the data from the remote \seqworkers to collocate them on the executor machine. This is an extremely expensive operation that defeats the major selling points of lazy blockchains: the separation between data dissemination and consensus. Furthermore, this execution machine needs to operate and persist the entire state of the system, introducing (i) an I/O bottleneck since the state does not fit in the main memory and (ii) a storage bottleneck since most machines only have a couple of drives mounted.
% One path to a solution would be the use of execution sharding~\cite{stefoexecuting}. Since transactions are already ordered it no longer suffers the security challenge, as a $51\%$ majority of honest per shard is sufficient. Nevertheless, the issues of adaptive security and state fragmentation still persist.

% How our approach fixes these shortcomings
This paper introduces \sysname, the first blockchain execution engine providing full elastic scalability,
tackling both the problems of remote data retrieval and distributed execution without compromising the security and simplicity of the system.
It is specifically designed for lazy blockchains and allows each validator to harness multiple machines under its control to scale its execution layer. These machines are potentially different from the \seqworkers used by lazy blockchains to store and disseminate transaction data and are named \emph{\execworkers}. Specifically, given a sufficiently parallelizable load, the number of transactions that the validator can execute with \sysname increases linearly with the number of \execworkers.
% As a result, existing systems fail to handle high throughput in real workloads. They are essentially monolithic wrappers loading all transactions data and executing them by calling a virtual machine, such as the Ethereum virtual machine (EVM)~\cite{evm} or the Move VM~\cite{move-vm}. The EVM is reported to peak at only 20k transactions per second when executing simple transactions (without JIT) and neglecting the retrieval of transaction data~\cite{evm-perf-1, evm-perf-2}, which also matches our benchmarks of the MoveVM. 
% These numbers are significantly lower than the throughput of the underlying blockchain, reaching over 100k even in large geo-distributed deployments~\cite{narwhal, bullshark, mysticeti, dumbo-ng}.
%
\sysname is inspired from traditional state sharding techniques, but the sharding is internal to the validator. Each \execworker handles a subset of the state, executes only a subset of the transactions, and contributes its compute and memory to the overall execution engine. As a result, for a compute-heavy workload, \sysname can scale execution from $2.5$k to $20$k transactions per second while maintaining the latency to $50$ms by scaling the number of \execworkers from $1$ to $8$. To design \sysname we had to overcome three core challenges.

% Key challenges and insights of our approach
First (i), \sysname requires a mechanism to efficiently fetch transactions from the \seqworkers and dispatch them for execution to the appropriate \execworkers, without compromising latency or throughput. Existing execution engines do not tackle this problem and simply load all transactions on a single executor machine~\cite{sui-lutris}. The use of sharding additionally means that the state is split across multiple machines and needs to be dynamically loaded to the location execution is planned to happen. Unlike existing sharded databases, this dynamic loading needs to happen deterministically in order to prevent blockchain forks. Recall that blockchains needs to provide serializability~\cite{serializability} for transactions and linearizability~\cite{linearizability} for object accesses, invariants much stronger than the usual snapshot isolation databases require.
To provide these guarantees, we bypass the consensus/execution abstraction layer and use the highly-available commit sequence as the ground truth for the dependencies transactions should respect, leading to a consistent execution state across validators.

Secondly (ii), \sysname needs to tolerate some \seqworkers and \execworkers crashing and recovering. Existing systems leverage various caching and MVCC techniques~\cite{bernstein1983multiversion} that do not naturally generalize to the setting in which \sysname operates. \sysname needs to handle partial crash-recovery, where each \seqworker or \execworker may crash and recover at a different pace than the others. \sysname thus needs to maintain enough state among \execworker as \emph{checkpoints} to allow recovering machines to catch up with the rest. A simple solution would be to resort to strong (and expensive) consensus-based replication techniques among workers internal to the validator~\cite{calvin,lamport2001paxos,ongaro2015raft}. However \sysname avoids such overhead by observing that consistency and availability of the commit sequence are already provided by the blockchain protocol. Thus, \sysname optimistically does lightweight, best-effort replication between workers, and relies on heavyweight recovery from other validators only if the optimistic replication fails.

Finally (iii), \sysname aims to support a simpler programming model where the transactions partially specify the input read and write set (e.g., as required for Move~\cite{sui-move}). This, however, creates an additional challenge for \sysname, as objects that might be accessed dynamically can be located in different \execworkers, meaning that we cannot overwrite them until all previous transactions have finished, effectively reverting back to sequential execution. Thus, in essence, enforcing write-after-write dependencies to be respected. %This would limit the parallelizability of the workload. 
\sysname circumvents this issue by leveraging its enforced determinism. Meaning that in-memory execution can be lost and safely recovered in the event of crashes. \sysname relies on a novel versioned-queue scheduling algorithm that allows for transactions with write-after-write conflicts to execute concurrently. We couple this with our crash recovery mechanism, in which only consistent states are persisted. As a result, upon a crash, \sysname simply needs to re-execute a few transactions, but thanks to the deterministic nature of the blockchain this does not pose any inconsistency risks.

We evaluate \sysname by studying its latency and throughput, while varying the number of \execworkers, the computational intensity, and the degree of contention of the workload.
We find that \sysname scales linearly to at least $8$ \execworkers when the workload is compute-bound, and to $4$ \execworkers when the workload is not compute-bound.
We find that \sysname has good scalability to at least $8$ \execworkers in all tested workloads; if the workload is compute-bound, then \sysname has linear scalability.
% We compare \sysname against a non-scale-out Sui~\cite{sui-lutris} baseline and find that \sysname matches or exceeds the performance of the baseline even when running on a single machine, and then continues to outperform the baseline by up to $8\times$ when running on $8$ \execworkers.

% Summary of contributions
\para{Contributions}
We make the following contributions:
\begin{itemize}
    \item We present \sysname, the first blockchain execution engine unlocking full elastic blockchain scalability.
    \item We extend \sysname to tolerate \execworker crash-faults and recover efficiently. Our fault-tolerance mechanism avoids the use of expensive inter-worker consensus-based replication, instead relying on lightweight, best-effort replication.
    \item We extend \sysname to support dynamic reads and writes, thus eliminating the limiting assumption that the input read and write set must be fully specified and supporting richer programming models.
          %where the input read and write set is only partially specified.
    \item We formally prove the serializability, linearizability, and liveness of \sysname, even in the presence of faults.
    \item We implement \sysname and empirically demonstrate its scalability through a rigorous evaluation under varying system loads.
\end{itemize}

==> sections/security.tex <==
\section{Security Arguments} \label{sec:security}
We intuitively argue that \sysname satisfies the properties of \Cref{sec:properties}. 
\ifpublish
Appendices~\ref{sec:proofs}, \ref{sec:recovery-proofs} and \ref{sec:child-proofs} provide formal proofs.
\else
Our full paper~\cite{fullversion} provides formal proofs.
\fi

\subsection{Security of the Base \sysname Protocol} \label{sec:base-protocol-proof-intuition}
We informally argue the security of the base \sysname protocol presented in \Cref{sec:design}. 
\ifpublish
The full proof can be found in Appendix~\ref{sec:proofs}.
\fi

\para{Serializability}
Intuitively, this property states that \sysname executes transactions in a way that is equivalent to the sequential execution of the transactions, as it comes from consensus\xspace
\ifpublish
(\Cref{def:sequential-schedule} of Appendix~\ref{sec:proofs})
\fi. The proof leverages the following arguments: (i) \sysname builds the pending queues $\pendingdb$ by satisfying the transaction dependencies dictated by the consensus protocol (i.e., the sequential schedule), (ii) \sysname accesses objects in the same order as the sequential schedule, and (iii) \sysname executes transactions in the same order as the sequential schedule.

\para{Determinism}
We argue that \sysname satisfies the determinism property (\Cref{def:determinism} of \Cref{sec:properties}). Intuitively, this property ensures that all correct validators have the same object state after executing the same sequence of transactions. The proof follows from the following arguments: (i) all correct \sysname validators build the same dependency graph given the same input sequence of transactions; (ii) individual transaction execution is a deterministic process\xspace
\ifpublish
(\Cref{as:deterministic-execution})
\fi; 
(iii) transactions explicitly reference their entire read and write set\xspace
\ifpublish
(\Cref{as:explicit-read-write-set})
\fi; 
and (iv) all validators executing the same transactions obtain the same state.

\para{Liveness}
We argue that \sysname satisfies the liveness property (\Cref{def:liveness} of \Cref{sec:model}). Intuitively, this property guarantees that valid transactions
\ifpublish
(\Cref{def:valid-transaction})
\fi are eventually executed. The proof argues that (i) all transactions are eventually processed\xspace
\ifpublish
(\Cref{def:processed-transaction}, see Appendix~\ref{sec:proofs})
\fi, and (ii) among those transactions, valid ones are not aborted.

\subsection{Modifications for Crash Recovery}
We modify the above arguments to show that \sysname satisfies the security properties defined in \Cref{sec:design} despite the crash-failure of $f_e$ out of $2f_e+1$ \execworkers in all shards.

\para{Serializability and Determinism}
\ifpublish
Appendix~\ref{sec:recovery-proofs} 
\else
The proof~\cite{fullversion}
\fi
argues both the serializability and determinism of the protocol by showing that \execworkers process the same input transactions regardless of crash faults. That is, no \execworker skips the processing of an input transaction or processes a transaction twice. The proof follows from the following observations: (i) \execworkers persist watermarks of the last transaction they successfully executed (as specified by the serial schedule). These watermarks, together with the knowledge of the commit sequence, prevent them from re-executing old transactions upon recovery. (ii) 
\ifpublish
Appendix~\ref{sec:recovery-proofs} 
\else
The proof
\fi
shows that there always exists at least one correct \execworker holding enough information to allow crash-recovering \execworkers to synchronize. This information either takes the form of checkpoints or buffered messages (see \Cref{sec:cft}).

\para{Liveness}
The liveness argument relies on the completeness of an eventually strong failure detector~\cite{chandra1996, crash-recovery-fd}.
Intuitively, a correct \execworker $w$ eventually detects the failure of a peer $x$, and performs the recovery procedure 
\ifpublish
(\Cref{alg:line:recover} of \Cref{alg:recovery}, see Appendix~\ref{sec:recovery-algorithms})
\fi to find another correct \execworker of shard $s$ to replace $x$.
% Because the number of failures in the system is bounded, $w$ performs this recovery procedure a bounded number of times when the failure detector eventually becomes strongly accurate.
\ifpublish
Appendix~\ref{sec:recovery-proofs}
\else
The proof~\cite{fullversion}
\fi thus argues the liveness property by showing that the recovery procedure 
\ifpublish
presented at \Cref{alg:line:recover} of \Cref{alg:recovery}
\fi
eventually succeeds. The protocol then resumes normal operation, and the liveness of the system follows from the that of the normal operation protocol (\Cref{sec:base-protocol-proof-intuition}).

\subsection{Modifications to Support Dynamic Objects}

We finally argue that the algorithm modifications for dynamic object accesses described in 
\ifpublish
\Cref{sec:dynamic,sec:child-algorithms} 
\else 
\Cref{sec:dynamic}
\fi 
do not break the serializability, determinism, and liveness properties defined in \Cref{sec:properties}.

\para{Serializability and determinism}
The main proof modifications arise from the fact that 
\ifpublish
\Cref{as:explicit-read-write-set} (Appendix~\ref{sec:proofs}) is not guaranteed in the modified dynamic reads and writes algorithm. That is,
\fi
transactions do not always entirely specify their read and write sets.
%
Intuitively, \sysname prevents the processing of conflicting transactions until all dynamic objects are discovered. This limits concurrency further than the base algorithms\xspace
\ifpublish
presented in Appendix~\ref{app:algorithms}, but Appendix~\ref{sec:appendix-split-queues} shows 
\else 
, but we describe~\cite{fullversion}
\fi
how to alleviate this issue by indexing the queues $\pendingdb[\cdot]$ with versioned objects, that is, tuples of $(\objectid, version)$, rather than only object ids.

\para{Liveness}
\ifpublish
\Cref{lm:eventual-processing} of Appendix~\ref{sec:proofs} assumes that all calls to $exec(\tx, \cdot)$ are infallible. However, supporting dynamic objects requires us to modify \Cref{alg:process-ready} as indicated in \Cref{alg:process-ready-child} and make the call $exec(\tx, O)$ fallible. Appendix~\ref{sec:child-proofs} proves that this change does not compromise liveness since all dynamically accessed objects are eventually discovered, and thus all calls to $exec(\tx, \cdot)$ eventually succeed.
\else
The base algorithms assume that all calls to $exec(\tx, \cdot)$ are infallible. However, supporting dynamic objects requires us to modify this and make the the call $exec(\tx, O)$ fallible. Our proof~\cite{fullversion} shows that this change does not compromise liveness since all dynamically accessed objects are eventually discovered, and thus all calls to $exec(\tx, \cdot)$ eventually succeed.
\fi
